Interactive Segmentation of Radiance Fields

Radiance Fields (RF) are popular to represent casually-captured scenes for new view synthesis and several applications beyond it. Mixed reality on personal spaces needs understanding and manipulating scenes represented as RFs, with semantic segmentation of objects as an important step. Prior segmentation efforts show promise but don't scale to complex objects with diverse appearance. We present the ISRF method to interactively segment objects with fine structure and appearance. Nearest neighbor feature matching using distilled semantic features identifies high-confidence seed regions. Bilateral search in a joint spatio-semantic space grows the region to recover accurate segmentation. We show state-of-the-art results of segmenting objects from RFs and compositing them to another scene, changing appearance, etc., and an interactive segmentation tool that others can use. Project Page: https://rahul-goel.github.io/isrf/

==> src/sections/4_implementation.tex <==
% \section{Implementation Details}
% {    
%     \label{sec:method}
%     All the methods propsoed have been implemented in PyTorch [cite pytorch] branching off the code provided by DVGOv2 [cite arxiv of dvgov2]. For K Means clustering we use FAISS (cite it). The experiments are run on a machine with RTX 2080Ti and 128 GB RAM.
    
%     The threshold for high confidence region is chosen manually (interactively and with ease) for each scene since it depends on the feature distribution of that scene.
%     The value of $\lambda$ chosen for teacher-student training is fixed at $0.001$.
%     The threshold $\tau$ used for region growing after bilateral filtering is fixed at $0.2$ for all scenes.
%     The kernel size for bilateral filter is 3 while the metric for spatial distance across voxels is Chebyshev distance. The bilateral filter runs with a padding of 1 for extending the borders and a stride size of 1, thus effectively resulting in the same sized grid. The values of $\sigma_f$ and $\sigma_d$ are both fixed to be $5.0$ for all scenes and experiments.
% }

\section{Implementation Details}
{
    All the methods proposed in the paper have been implemented using PyTorch [cite pytorch] branching off the code provided by DVGOv2 [cite dvgov2]. The experiments have been run on NVIDIA RTX 2080Ti.
    
    The components of the radiance fields namely the volumetric density, radiance latent vectors and the learnt DINO features have all been stored using VM decomposition proposed by TensoRF [cite tensorf]. For radiance latent vectors, we use VM-48 representation and for DINO features, we use VM-64 representation. The segmentation masks have been stored as a 3D bitmap.
    
    The DINO ViT-b8 model provides 768 features for each patch of 8x8 pixels in an image. We reduce the dimension of the features by taking a 64 dimensional PCA for all the features across each image. For each pixel, the feature is calculated by referring to the feature of the patch that pixel lies in.
    
    We pre-train the model for the volumetric density and radiance for $20,000$ epochs. We introduce distillation using student-teacher training with $\lambda = 0.001$ for the weighted loss function for $5,000$ epochs. The loss is taken on the features and radiance together to maintain consistency.
    
    We choose $K = 10$ when applying K-Means to the set of features selected from the user's brush stroke. For the bilateral filter, the value of $\sigma_\phi$ and $\sigma_s$ are both set to $0.5$ and the value of the threshold $\tau$ is $0.2$.
}

\section{Scene Editing}
{
    In this section, we explain the procedures we followed for editing the 3D scenes post segmentation. The segmentation procedure provides a 3D bit map representing the segmented voxels.
    
    \subsection{Object Removal}
    {
    For removing a segmented object from the scene, we alter the evaluation of the density for a 3D point. We simultaneously evaluate the bit map value $b_x$ at the queried point. To remove the segmented object, the effective density $\sigma'_x$ is replaced by $\sigma_x * (1.0 - b_x)$
    }
}

==> src/sections/OldIntro.tex <==
\section{Introduction}
{
    \label{sec:intro}
    
    \begin{itemize}\itemsep=0mm
    \color{blue}{
        \item Abstract: ends at 2/3rd of the first colum
        \item Intro: ends at the bottom of first column, second page. (Diagram also there)
        \item Related work: 2/3rd col on page 2 plus one full column on page 3
        \item Section 3 (method) starts top of second col on page 3. Goes till end of first col on page 4
        \item Section 4: Half a column. Now we have filled 4.75 pages. We have 3.25 pages left
        \item Results section: 1 full column of text
        \item Tables 1 col width, 1/3 col height.
        \item Images: 4 rows of images with full width. Fills 3/4th of a page
        \item Interactive segmentation imaage: 1/4th of a page
        \item Ablation with images: 0.5 pages 
        \item Discussion, Conlusion, Limitation: 0.5 page
        }
        \item {\color{red}WE SHOULD TAKE ABOUT HIGH CONFIDENCE AND GROWING IN INTRO}
    \end{itemize}
    
    Scene representation is a crucial step prior to any scene understanding or manipulation task. Relevant scene parameters, be it shape, appearance or illumination, can be represented using a variety of modalities like $2$D (depth/texture) maps, point clouds, surface meshes, voxels, parametric functions \etc. Each modality facilitates some task while taxing some other aspect of the process. For example, shape correspondence is straightforward between point clouds compared to surface meshes but compromises on rendering fidelity. Thus, choosing an appropriate representation has a major effect on the downstream 3D analyses and applications.
    
    Neural implicit representations, which parameterize object surface as a zeroth level-set of a volumetric function, have emerged as most promising modality for 3D analysis. Although initially proposed only for shapes \cite{SDF,Occupancy}, such representation have been extended to encode complete directional radiance at a point \cite{nerf} and even beyond the basic rendering parameters to lightfields, specularity, audio, textual context, object semantics, \etc \cite{nerf+lightfeld, nerf+specular, nerf+audio, nerf+text, nerf+semantics}. Subsequent works have focused on addressing the observed short-comings in the pioneering methods like high training/rendering time, high computational overhead, requirement of numerous multiview images, scene specific training, inefficient storage, complex rendering process, \etc. Apart from such efficiency improvements, there is an ongoing research on extending these representations beyond the simpler static inward-looking and front-facing scenes to more complex outwards-looking unbounded $360^{\circ}$ views, dynamic clips, heavily occluded egocentric videos and unconstrained images acquired \textit{in-the-wild}.
    
    Although, initially targeted at Novel View Synthesis (NVS), now the radiance field research has exploded beyond it into several other application fields like \cite{}, \cite{} \etc. This has led back to the merger of implicit representations with the traditional 3D modalities like point clouds, surface meshes, voxels and 2D maps, as necessitated by the focal application. This has led to the proposition of several hybrid implicit-explicit representations like \cite{} which aim to harness the advantages of both the strategies. Unlike implicitly MLP-encoded representations like NeRF, which are not easily amenable, such hybrid representations enable simpler employment in the downstream applications with an additional benefit of further improved quality and efficiency.
    
    One such interesting and challenging application is controlled radiance field manipulation by either editing the existing content or by compositing new objects into the scene. Most of the direct editing solutions show results by either retraining from scratch for composition \cite{} or performing post-hoc edits on the depth buffers from the rendered views \cite{}. This workflow is inflexible in a real world usage scenario and does not efficiently harness the scene information from the representation thereby affecting the quality of the final edited results.
    Yet another way to perform basic scene understanding and semantic segmentation as the initial steps which pose a challenging task by themselves.
    The former needs to be extracted from the encoded geometric information in the radiance fields and the latter can be assisted via user-provided annotations, textual cues or prelearnt priors.
    Though the aforementioned methods thrive in the generation of novel views, little has been done in the direction of scene understanding specifically object segmentation. Recently, N3F \cite{} and DFF \cite{} have proposed solutions to this end but make use of Neural Space for the Radiance Field representation, which complicate the editing process. Both are fundamentally similar in the underlying intuition of using distillation for feature matching between user provided cues  with the learned 3D feature volume. A minor difference is that N3F uses patches whereas DFF employs textual prompts as the segmentation cues. Segmentation is often a tedious iterative task, and user interactivity is a highly desirable trait in such an application. Both N3F and DFF do not directly support interactivity and facilitating it in the Neural space is a difficult undertaking. 
     
    In this work, we address the shortcoming of the two prior works while proposing a simple yet efficient method which outperforms both the methods while achieving fine-grain details. We present an interactive and intuitive framework for radiance field manipulation. The basic idea underlying our proposed method is the appropriate selection between the relevant representations for the given task at hand and gradual iterative refinement from a high confidence seed. Specifically, we interchangeably employ factorized-tensor \ie TensoRF \cite{} and encoded voxel-grid \ie DVGO \cite{}, hybrid representations in our framework. TensoRF allows faster training and rendering with lower storage overhead whereas DVGO enables simpler manipulation operations directly on a 3D lattice. Overall, this leads to easy yet higher quality scene manipulations like object- segmentation, removal, appearance stylization, replacement and novel view synthesis, even using simple traditional 3D editing techniques. In summary, following are our core contributions:
    \begin{itemize}[label={$\circ$}]
    \itemsep0ex
        \item We provide an easily interpretable yet qualitatively improved object segmentation framework for radiance field manipulation. 
        \item Our method allow the user to interactively modify the desired regions from the segmented results thereby enabling a more natural editing workflow.
        \item Our proposed method is based hybrid implicit-explicit representation using using which we effectively harnesses the geometric and distilled semantic information for improved segmentation results. Our results show improved accuracy and fine-grain object details compared to the contemporary SOTA.
        \item We show qualitative and quantitative segmentation comparisons on multiple scene types and usage on several downstream applications like NVS, appearance alteration, object replacement \etc.
        % \item We present a simple yet useful way of fusing the new composition into a compact TensoRF representation.
    \end{itemize}
    }

    % \doit[inline]{talk about distillation , transformer features ?}
    % \hline
    % Scene understanding and scene manipulation have been the interest of the community lately. The task of understanding and manipulation often requires the AUTHORING OF SCENES in geometric software like Blender[CITE BLENDER UNITY], Unity, etc. With the advent of high-resolution image capture cameras in handheld mobile phones, a vast number of high-quality image priors are available for augmenting geometric authoring(cite Voxel coloring steive sitz, dynamic fusion). Of late methods like Neural Radiance Fields DUBBED as NeRFs [CITE nerfs as many as possible nerf mip nerf nerfplusplus] have demonstrated enormous potential in utilizing simple MLPs to encode the whole scene while understanding geometry and radiance from a set of discrete image inputs. The follow-up works have exploited the Voxel spaces to speed up the process of representing Radiance fields[CITE Plenoxels, TensoRF, DVGO].

    % Though the aforementioned methods thrive in the generation of Novel views, little has been done in the direction of scene understanding specifically object segmentation. 
    % --> The works like DFF, N3F, D2NeRF[CITE concerned papers] try to understand specific objects from the scene at hand to facilitate object separation. {\color{red} Saurabh Sir: DFF and N3F learn a feature field using teacher-student model utilizing DINO}. Both N3F and DFF make use of Neural Space for the Radiance Field representation, which limits the object query space largely (See Sec.[refer to the section explaining the patch etc.]). Additionally, the works also suffer in obtaining fine-grain details(Ribs of T-Rex) and hold DINO accountable for it[CITE DFF].
    % --> Segmentation is often a tedious task, and interactivity is a highly desirable trait. Both DFF and N3F do not support interactive segmentation and facilitating it in Neural space is not a viable solution.

    % In this work, we address the shortcoming of the prior work while proposing a method simple yet efficient method which outperforms both prior methods while achieving fine-grain details.
    % --> We do this without the usage of any semantic supervision of the scene while adhering to the widely used DINO similar to that of DFF and N3F. During our study, we found that traditionally available and tested approaches like Bilateral Filtering, Voxel growing, and NNFM will augment the segmentation vastly incorporating finer details. We also facilitate interactive addition and removal of desired and undesired content from the scene which is one of the major caveats in the prior.
    
    %  To achieve this we {\color{red} Saurabh Sir: build up the method of Distillation similar to that of DFF and N3F conditioned on DINO features}. Unlike the prior art, we exploit the Voxel space more specifically compressed Voxel space like [cite TensoRF] for the distillation. We rely on meticulously tested and explored traditional methods like Bilateral Filtering, Voxel growing, and NNFM to segment the object accurately. Along with these we also facilitate interactive addition and removal of desired and undesired content.  

    % [Add more details here sparely here make it clear that fine grain does not mean hair-level shit, specify that we are only using SSL DINO + NeRF no input labeled data]
 

==> src/sections/selfNotes.tex <==
 \section{notes}
 {
      %   \label{sub_sec:notes}
      %   \begin{itemize}\itemsep=0mm
      %       \item Results for the paper+supplementary: Which scenes?•Which are the new scenes?
      %       \item Additional Experiments (Ablations, etc.): What are the other design choices that we can include?Results for the 
      %       \item Video: A few scenes Which are the good scenes to show? Interactive segmentation: Positive and negative strokes, object getting segmented, shown by moving around
      %       \item Let us plan this quickly Need not be live. 
      %       \item  Show snapshots at different times
      %       Segmentation of a difficult scene like Dinosaur.
      %       \item And something in 360 degree view with fine structure like Dinosaur
      %       \item Fusion results
      %       \item Resegmentation after fusion to prove proper fusion
      %       \item Add another plant to an existing flower-pot and fuse it 
      %       Later, select the pot again and the whole thing gets selected
      %       \item What else?(Question: Do we have one more week for the video? But, we need to show some of those results in the paper also)
      %   \end{itemize}
        
        
      %   \begin{itemize}\itemsep=0mm
      %       \color{red}{
      %           \item Results on 8 LLFF scenes. {\em Done. \bf Main: Big differences (stove, shoerack, chess table, ...). Suppl: Remaining with lower differences}
      %           \item 4 360V2 scenes {\em 2 done for main paper. \bf Strokes, both +ve \* -ve. Growing with BLF. Editiing to bring lego to table. \\
      %           Apperance editing (stylization of the pot, lego. Supplementary: More results}
      %           \item Baselines: N3F {\em Trained, results to be taken. \bf Results taken!!\\
      %           \bf Comparison: Patch given as input to both methods. 4 examples, 3 cols each. Big difference will be shown. Suppl: More examples
      %           }
      %           \item Variants: Average, NNFM, NNFM+Kmeans, Bilater Filtering {\em Data is available for the main paper.\\
      %           \bf Main paper: Ablations. All of above using strokes only. No comparison. Supplementary: More examples
      %           }
      %           \item Metrics MeanIOU, mAP, {\em Not sure how to do. To figure out with Saurabh. Plan: Do 2 ScanNet scenes for main paper. Do 10-20 scenes (or as many as possible) for suppl}
      %           \item 2D Baseline Video (Temporal Segmentation SEGNet) IVOS Sanja fidler. {\em Do this only for Supplementary?? Lowest priority main paper. Is this required at all?}
      %           \item short term and long term consistency. in 2D {\em Warp segmented objects from frame i to frame j. Compare in 3D space? Or rendered image space? Using optical flow? This is strongly for supplementaty!??}
      %           \item Appearance editing sub-scene segmentation, stylization {\em Stylize segmented object only. Relearn MLP. Rendering into background using Z-buffer. \bf Suppl: More results}
                
      %           \item Figures
      %           \item Teaser
      %           \item Method Diagram {\bf To be done. Sketch with S. R will do}
      %           \item Segmentation (all the variants and ours vs N3F) {\em Data is available. \bf For Supplementary}
      %           \item Interactive display of segmentation (time growing) {\em Older results done. Can do more.\bf Some pictures in Main paper. Rest suppl/video}
      %           \item Editing (Removal, appearance change, translation, unifrom rescale) {\em Removal done. Others to be done. \bf Some in main paper. Rest in suppl}
      %           }
            
      %  %    \color{green}{\item N3F all trained, needs fine tune for the}
            
      %   \end{itemize}
      % }   
      % }
      
      % \subection{\large\bf Things to put in the supplementary}
    \textcolor{red}{
        \begin{itemize}      
        \item Show removal of multiple objects in the garden scene: pot, tabletop, steelballs
            \item Make Replica run with our codebase. Select some non-blurry scenes. Calculate the segmenation metrics and report in table.
            \item Show multiple positive/negative stroked results. This is on the garden scenes as well as some more LLFF scenes.
            \item Get additional results on more LLFF scenes. Instead of using a lot of scenes, it would be better to show segmentation of different objects in the same scene. (All stroke based.) Scenes are not decided yet.
            \item Make a video of the results. (Good segmentations and stroke based segmentation results.) Choose the results generated above.
            \item Make a video about the method. (Dhawal)
            \item For editing of scenes, mention the procedure used. Set sigma to 0 for removal, introduce ray-point query shift for translation, etc.
            \item How union and intersection is done to incorporate positive and negative strokes.
        \end{itemize}
        }
    \textcolor{green}{
        \begin{itemize}
            \item Hand-annotate for the 4 scenes of LLFF and show the metrics.
            \item There are lots and lots of implementation details. Make sure to mention all of them in a clean and clear manner.
            \item Show multiple instances progressive editing on the garden + JCB scene. Show original garden scene, remove the pot, put JCB under table (it is the default position when I try to do composition), move it to the table, apply style to it. NOT PUTTING IT UNDER DUE TO LACK OF HORIZONTAL SPACE + IT DOESN'T LOOK GOOD.
            \item Show difference between learnt teacher and student DINO features and show how the student surpasses the teacher.
            \item Show ribcages of T-Rex getting segmented but the tail failing. State the reason behind that.
        \end{itemize}
    }
}

